Automatic Generation of Multiple-Choice Questions

Creating multiple-choice questions to assess reading comprehension of a given article involves generating question-answer pairs (QAPs) and adequate distractors. We present two methods to tackle the challenge of QAP generations: (1) A deep-learning-based end-to-end question generation system based on T5 Transformer with Preprocessing and Postprocessing Pipelines (TP3). We use the finetuned T5 model for our downstream task of question generation and improve accuracy using a combination of various NLP tools and algorithms in preprocessing and postprocessing to select appropriate answers and filter undesirable questions. (2) A sequence-learning-based scheme to generate adequate QAPs via meta-sequence representations of sentences. A meta-sequence is a sequence of vectors comprising semantic and syntactic tags. we devise a scheme called MetaQA to learn meta sequences from training data to form pairs of a meta sequence for a declarative sentence and a corresponding interrogative sentence. The TP3 works well on unseen data, which is complemented by MetaQA. Both methods can generate well-formed and grammatically correct questions. Moreover, we present a novel approach to automatically generate adequate distractors for a given QAP. The method is a combination of part-of-speech tagging, named-entity tagging, semantic-role labeling, regular expressions, domain knowledge bases, word embeddings, word edit distance, WordNet, and other algorithms.

==> abstract.tex <==
% \begin{abstract}
Creating multiple-choice questions to assess reading comprehension of a given article involves generating question-answer pairs (QAPs) and adequate distractors. 
%We tackle this challenge by dividing it into two tasks: question generation and distractor generation. 
We present two methods to tackle the challenge of QAP generations:
(1) A deep-learning-based end-to-end question generation system based on T5 Transformer with Preprocessing and Postprocessing Pipelines (TP3).
We use the finetuned T5 model for our downstream task of question generation and improve accuracy using a combination of various NLP tools and algorithms in preprocessing and postprocessing to select appropriate answers and filter undesirable questions.
(2) A sequence-learning-based scheme to generate adequate QAPs via meta-sequence representations of sentences.
A meta-sequence is a sequence of vectors comprising semantic and syntactic tags. we devise a scheme called MetaQA to learn meta sequences from training data to form pairs of a meta sequence for a declarative sentence and a corresponding interrogative sentence.
% A trained MetaQA model converts a given declarative sentence to a meta sequence, finds a matched MD, and uses the corresponding MIs and the input sentence to generate QAPs. 
The TP3 works well on unseen data, which is complemented by MetaQA. 
Both methods can generate well-formed and grammatically correct questions.
Moreover, we present a novel approach to automatically generate adequate distractors for a given QAP. The method is a combination of part-of-speech tagging, named-entity tagging, semantic-role labeling, regular expressions, domain knowledge bases, word embeddings, word edit distance, WordNet, and other algorithms. 
% \end{abstract}

==> acknowledgements.tex <==
\chapter*{Acknowledgments}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\hspace{\parindent}
I would like to express my sincere gratitude to my advisor Dr. Jie Wang for his continuous support of my Ph.D study and research. 
His motivation, insights, patience, and immense knowledge guided my research and the writing of this dissertation.

I would also like to thank Dr. Yu Cao and Dr. Karen Lin to serve on my thesis committee. 
I am grateful to their insightful suggestions and encouragement.

I thank my fellow labmates Hao Zhang, Yicheng Sun, Changfeng Yu and You Zhou for their stimulating discussions and collaborations on a number of projects throughout my studies.

I would also like to thank the faculty and staff
% and my colleagues 
at the Computer Science department of UMass Lowell, many people have helped me not just in research effort, but in introducing me to new thoughts and ideas.

Last but not least, I am indebted to my family for supporting me spiritually throughout my life.

==> bibliography.tex <==
%% This defines the bibliography file (main.bib) and the bibliography style.
%% If you want to create a bibliography file by hand, change the contents of
%% this file to a `thebibliography' environment.  For more information 
%% see section 4.3 of the LaTeX manual.
\bibliographystyle{apalike}
%\bibliographystyle{abbrvnat-quote}
%\bibliographystyle{plainnat}
\renewcommand{\bibname}{References}
\bibliography{bibliography}


==> biography.tex <==
\chapter{Publications}

% As of 2012, UMass Lowell calls for a ``Biographical Sketch of Author.''

% The required brief biographical sketch should include the names of schools attended, the exact designation of diplomas and degrees awarded, the title and nature of any post-collegiate employment, together with the name and location of the employing organization, and a description of any previous graduate study or related research, publications, or special professional interests.


==> chapter_template.tex <==
\chapter{Introduction}

\section{Problem statement}

\section{Approach}

\section{Research contributions}

\section{Outline of the thesis}


==> preface.tex <==
\chapter*{Preface}
The preface is not part of the thesis standard, but is optionally available if you find it prudent. Uncomment it in main.tex.


==> publication.tex <==
\nociteNew{*}
\bibliographystyleNew{apalike}
%\bibliographystyle{abbrvnat-quote}
%\bibliographystyle{plainnat}
\renewcommand{\bibname}{Publication}
\bibliographyNew{publication}

